Why Do Students Lie and Should We Worry? An Analysis of Non-truthful Reporting

A core aspect in market design is to encourage participants to truthfully report their preferences to ensure efficiency and fairness. Our research paper analyzes the factors that contribute to and the consequences of students reporting non-truthfully in admissions applications. We survey college applicants in Denmark about their perceptions of the admission process and personality to examine recent theories of misreporting preferences. Our analysis reveals that omissions in reports are largely driven by students' pessimistic beliefs about their chances of admission. Moreover, such erroneous beliefs largely account for whether an omission led to a missed opportunity for admission. However, the low frequency of these errors suggests that most non-truthful reports are "white lies" with minimal negative impact. We find a novel role of personality and individual circumstances that co-determine the extent of omissions. We also find that estimates of students' demand are biased if it is assumed that students report truthfully, and demonstrate that this bias can be reduced by making a less restrictive assumption. Our results have implications for the modeling of preferences, information acquisition, and subjective admission beliefs in strategy-proof mechanisms

==> tables/2020_udgaver/clogit_res.tex <==
\begin{table}[htbp]
\centering
\small
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
            &\multicolumn{1}{c}{Revealed Pref}&\multicolumn{1}{c}{Stated Pref}&\multicolumn{1}{c}{Stated Pref}&\multicolumn{1}{c}{Revealed Pref}&\multicolumn{1}{c}{Stated Pref}&\multicolumn{1}{c}{Stated Pref}\\
\hline
        &            &            &            &            &            &            \\
Distance (1000 km)&       -9.74&       -9.92&      -10.00&       -9.71&       -9.96&       -9.99\\
            &      (0.18)&      (0.18)&      (0.18)&      (0.18)&      (0.18)&      (0.18)\\
Program Peer Quality&        9.21&        7.12&        8.20&        9.43&       19.61&       15.70\\
            &      (0.10)&      (0.08)&      (0.09)&      (0.33)&      (0.43)&      (0.41)\\
Same Gender Share&        1.72&        1.62&        1.71&        2.26&        2.25&        2.27\\
            &      (0.04)&      (0.04)&      (0.04)&      (0.06)&      (0.06)&      (0.06)\\
Program Peer Parents Inc&        4.35&        2.70&        3.77&        4.66&        5.55&        5.82\\
            &      (0.21)&      (0.19)&      (0.19)&      (0.65)&      (0.64)&      (0.65)\\
\hline
N           &   6,888,528&   6,888,528&   6,340,871&   6,888,528&   6,888,528&   6,340,871\\
Program FE  &          No&          No&          No&         Yes&         Yes&         Yes\\
Stability Assumption&          No&          No&         Yes&          No&          No&         Yes\\
\hline\hline
\end{tabular}
\caption{Conditional Logit Regressions...}
\label{tab:XXXX}
\floatfoot{Notes: ...}
\end{table}


==> tables/2020_udgaver/clogit_res_2020.tex <==
\begin{table}[htbp]
\centering
\small
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
            &\multicolumn{1}{c}{Revealed Pref}&\multicolumn{1}{c}{Stated Pref}&\multicolumn{1}{c}{Stated Pref}&\multicolumn{1}{c}{Revealed Pref}&\multicolumn{1}{c}{Stated Pref}&\multicolumn{1}{c}{Stated Pref}\\
\hline
        &            &            &            &            &            &            \\
Distance (1000 km)&       -9.53&       -9.58&       -9.74&       -9.59&       -9.69&       -9.79\\
            &      (0.23)&      (0.23)&      (0.23)&      (0.24)&      (0.24)&      (0.24)\\
Program Peer Quality&        9.27&        7.14&        9.54&       11.07&       27.49&       12.34\\
            &      (0.14)&      (0.12)&      (0.15)&      (0.49)&      (0.87)&      (0.76)\\
Same Gender Share&        1.73&        1.61&        1.79&        2.26&        2.27&        2.29\\
            &      (0.06)&      (0.06)&      (0.06)&      (0.08)&      (0.08)&      (0.09)\\
Program Peer Parents Inc&        3.80&        2.26&        4.02&        8.28&       10.42&       10.65\\
            &      (0.30)&      (0.27)&      (0.25)&      (1.13)&      (1.15)&      (1.10)\\
\hline
N           &   3,771,368&   3,771,368&   3,224,261&   3,771,368&   3,771,368&   3,224,261\\
Program FE  &          No&          No&          No&         Yes&         Yes&         Yes\\
Stability Assumption&          No&          No&         Yes&          No&          No&         Yes\\
\hline\hline
\end{tabular}
\caption{Conditional Logit Regressions...}
\label{tab:XXXX}
\floatfoot{Notes: ...}
\end{table}


==> tables/2020_udgaver/lin_reg_res_FE.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\small
\renewcommand{\arraystretch}{1.25} 
\begin{tabular}{lcccc} \hline \hline
                                                            & \multicolumn{2}{c}{Reports non-truthfully} & \multicolumn{2}{c}{Skips the impossible} \\
                                                            & (1)             & (2)             & (3)           & (4)      \\  \hline
\textit{Academic achievements}                              &                 &                 &               &          \\                            
Eligibility score                                           & -0.0561         & -0.0513         & -0.0436       & -0.0411  \\
                                                            & (0.004)         & (0.004)         & (0.004)       & (0.004)  \\
Middle school GPA                                           &  0.0068         &  0.0074         &  0.0049       &  0.0047  \\
                                                            & (0.005)         & (0.005)         & (0.004)       & (0.004)  \\
\textit{Demographics}                                       &                 &                 &               &          \\
Age                                                         & -0.0022         & -0.0029         &  0.0007       & -0.0003  \\
                                                            & (0.003)         & (0.003)         & (0.002)       & (0.002)  \\
Female                                                      &  0.0187         & -0.0007         &  0.0032       & -0.0086  \\
                                                            & (0.014)         & (0.014)         & (0.019)       & (0.012)  \\
\textit{Socioeconomic factors}                              &                 &                 &               &          \\
Income percentile, parents                                  & -0.0440         & -0.0223         & -0.0162       & -0.0016  \\
                                                            & (0.029)         & (0.028)         & (0.024)       & (0.023)  \\
\textit{Self-stated covariates}                             &                 &                 &               &          \\
Confidence in own abilities                                 &                 & -0.0189         &               & -0.0095  \\
                                                            &                 & (0.003)         &               & (0.003)  \\
Risk profile                                                &                 &  0.0005         &               & -0.0012  \\
                                                            &                 & (0.003)         &               & (0.0027) \\
Pessimistic                                                 &                 &  0.0438         &               &  0.0560   \\
                                                            &                 & (0.013)         &               & (0.0115) \\
Failed anticipation of cutoff movement                      &                 &  0.0521         &               &  0.0296  \\
                                                            &                 & (0.030)         &               & (0.025)  \\     
\multirow{2}{5cm}{Willingness to postpone an additional year} &               & -0.0962         &               & -0.0692  \\
                                                            &                 & (0.014)         &               & (0.012)  \\
Perceive rejection as a failure                             &                 & -0.0043         &               & -0.0002  \\
                                                            &                 & (0.012)         &               & (0.010)  \\
\multirow{2}{5cm}{Difficult to comprehend admission process}&                 &  0.0270         &               &  0.0210  \\
                                                            &                 & (0.013)         &               & (0.011)  \\ \hline
Study program fixed effects                                 & Yes             & Yes             & Yes           & Yes      \\              
N                                                           & 4,128           & 4,128           & 4,128         & 4,128    \\ \hline \hline       
\end{tabular}
\caption{Coefficient Results of Linear Probability Models}
\label{tab:lin_reg_res_FE}
\floatfoot{Notes: The table shows results for four separate linear probability regression models. The table reports coefficient estimates and robust standard errors in parenthesis. Equation (1) and (2) consider non-truthful reporting as an outcome variable. Non-truthful reporting is defined as survey respondents who state they would change their submission if they could be enrolled at any study program. Equation (3) and (4) consider skipping the impossible as an outcome variable. Skipping the impossible is defined as survey respondents who state they would select a different first priority study program if they could be enrolled at any study program. The regressions are based on survey respondents for whom we have full data for. That is, survey respondents with missing data inputs are neglected in the regressions. Every equation include fixed effects for respondents' revealed first choice study program.}
\end{table}

==> tables/2020_udgaver/lin_reg_res_noFE.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\small
\renewcommand{\arraystretch}{1.25} 
\begin{tabular}{lcccc} \hline \hline
                                                            & \multicolumn{2}{c}{Reports non-truthfully} & \multicolumn{2}{c}{Skips the impossible} \\
                                                            & (1)                 & (2)                   & (3)              & (4)     \\  \hline
\textit{Academic achievements}                              &                     &                       &                  &         \\                            
Eligibility score                                           &   -0.0481           & -0.0416               & -0.0323          & -0.0291 \\
                                                            &   (0.004)           & (0.004)               & (0.003)          & (0.003) \\
Middle school GPA                                           &     0.0040          & 0.0050                &  0.0029          &  0.0037 \\
                                                            &   (0.005)           & (0.005)               & (0.004)          & (0.004) \\
\textit{Demographics}                                       &                     &                       &                  &         \\
Age                                                         &    0.0001           &  0.0000               &  0.0028          &  0.0028 \\
                                                            &   (0.003)           & (0.003)               & (0.002)          & (0.003) \\
Female                                                      &      0.0331         &  0.0146               &  0.0146          &  0.0047 \\
                                                            &    (0.012)          &  (0.012)              & (0.010)          & (0.010) \\
\textit{Socioeconomic factors}                              &                     &                       &                  &         \\
Income percentile, parents                                  &     -0.0335         &  -0.0113              & -0.0023          &  0.0118 \\
                                                            &    (0.027)          &   (0.027)             & (0.022)          & (0.022) \\
\textit{Self-stated covariates}                             &                     &                       &                  &         \\
Confidence in own abilities                                 &                     &  -0.0199              &                  & -0.0099 \\
                                                            &                     &  (0.003)              &                  & (0.003) \\
Risk profile                                                &                     &  0.0028               &                  &  0.0009 \\
                                                            &                     &  (0.003)              &                  & (0.003) \\
Pessimistic                                                 &                     &  0.0291               &                  &  0.0213 \\
                                                            &                     &  (0.012)              &                  & (0.010) \\
Failed anticipation of cutoff movement                     &                     &  0.0573               &                  &  0.0163 \\
                                                            &                     &  (0.029)              &                  & (0.023) \\                           
\multirow{2}{5cm}{Willingness to postpone an additional year} &                   &  -0.0941              &                  & -0.0642 \\
                                                            &                     &  (0.014)              &                  & (0.012) \\
Perceive rejection as a failure                            &                      &  0.0175               &                  &  0.0186 \\
                                                            &                     &  (0.012)              &                  & (0.010) \\
\multirow{2}{5cm}{Difficult to comprehend admission process}  &                   &  0.0359               &                  &  0.0314 \\
                                                            &                     &  (0.013)              &                  & (0.010) \\ \hline
Study program fixed effects                                 & No                  & No                    & No               & No      \\              
N                                                           & 4,128               & 4,128                 & 4,128            & 4,128   \\ \hline \hline       
\end{tabular}
\caption{Coefficient Results of Linear Probability Models (no fixed effects)}
\label{tab:lin_reg_res_noFE}
\floatfoot{Notes: The table shows results for four separate linear probability regression models. The table reports coefficient estimates and robust standard errors in parenthesis. Equation (1) and (2) consider non-truthful reporting as an outcome variable. Non-truthful reporting is defined as survey respondents who state they would change their submission if they could be enrolled at any study program. Equation (3) and (4) consider skipping the impossible as an outcome variable. Skipping the impossible is defined as survey respondents who state they would select a different first priority study program if they could be enrolled at any study program. The regressions are based on survey respondents for whom we have full data for. That is, survey respondents with missing data inputs are neglected in the regressions.}
\end{table}

==> tables/2020_udgaver/linreg_FE_nontruthful.tex <==
\begin{table}[]
\centering
\small
\renewcommand{\arraystretch}{1.25} 
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
 & \multicolumn{4}{c}{\textbf{Reports non-truthfully}} \\
 & (1) & (2) & (3) & (4) \\                               
\hline
\multicolumn{5}{l}{\textit{Self-stated admission beliefs, favorite program} } \\
States zero admission probability&       0.057\sym{*}  &                     &                     &       0.051\sym{*}  \\
            &     (0.023)         &                     &                     &     (0.024)         \\
Stated admission probability&      -0.003\sym{***}&                     &                     &      -0.002\sym{***}\\
            &     (0.000)         &                     &                     &     (0.000)         \\
\textit{Academic achievements}                             &                 &                 &               &          \\            
Eligibility score&                     &      -0.056\sym{***}&                     &      -0.025\sym{***}\\
            &                     &     (0.004)         &                     &     (0.005)         \\
Middle school GPA&                     &       0.007         &                     &       0.007         \\
            &                     &     (0.005)         &                     &     (0.005)         \\
\textit{Demographic}                             &                 &                 &               &          \\              
Age         &                     &      -0.002         &                     &      -0.004         \\
            &                     &     (0.003)         &                     &     (0.003)         \\
Female      &                     &       0.019         &                     &      -0.007         \\
            &                     &     (0.014)         &                     &     (0.014)         \\
\textit{Socioeconomic factors}                             &                 &                 &               &          \\              
Income percentile, parents&                     &      -0.044         &                     &      -0.029         \\
            &                     &     (0.029)         &                     &     (0.028)         \\
\textit{Self-stated covariates}                             &                 &                 &               &          \\                 
Confidence in own abilities&                     &                     &      -0.027\sym{***}&      -0.016\sym{***}\\
            &                     &                     &     (0.003)         &     (0.003)         \\
Risk profile&                     &                     &       0.009\sym{**} &      -0.001         \\
            &                     &                     &     (0.003)         &     (0.003)         \\
Pessimistic &                     &                     &       0.050\sym{***}&       0.036\sym{**} \\
            &                     &                     &     (0.013)         &     (0.013)         \\
Failed anticipation of cutoff movement&                     &                     &       0.092\sym{**} &       0.052         \\
            &                     &                     &     (0.029)         &     (0.030)         \\
Willingness to postpone an additional year&                     &                     &      -0.093\sym{***}&      -0.096\sym{***}\\
            &                     &                     &     (0.014)         &     (0.014)         \\
Perceives rejection as failure&                     &                     &       0.020         &      -0.004         \\
            &                     &                     &     (0.012)         &     (0.012)         \\
Difficult to comprehend admission process&                     &                     &       0.029\sym{*}  &       0.026\sym{*}  \\
            &                     &                     &     (0.013)         &     (0.013)         \\
\hline
N           &    4,402         &    4,128        &    4,402         &    4,128         \\
Study program fixed effects&         Yes         &         Yes         &         Yes         &         Yes         \\
\hline\hline
\end{tabular}
}
\caption{Coefficient Results of Linear Probability Models for Non-truthful Reporting}
\label{tab:lin_reg_res_FE_nontruthful}
\floatfoot{Notes: The table shows results for four separate linear probability regression models. The table reports coefficient estimates and robust standard errors in parenthesis. Each equation consider non-truthful reporting as an outcome variable. Non-truthful reporting is defined as survey respondents who state they would change their submission if they could be enrolled at any study program. Survey respondents with missing data inputs are neglected in the regressions. Every equation include fixed effects for respondents' revealed first choice study program. \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\).}

\end{table}

==> tables/2020_udgaver/linreg_FE_regretskip.tex <==
\begin{table}[]
\centering
\small
\renewcommand{\arraystretch}{1.25} 
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
 & \multicolumn{4}{c}{\textbf{Payoff relevant mistakes}} \\
 & (1) & (2) & (3) & (4) \\  
\hline
\multicolumn{5}{l}{\textit{Self-stated admission beliefs, favorite program} } \\
States zero admission probability&       0.011         &                     &                     &       0.011         \\
            &     (0.007)         &                     &                     &     (0.008)         \\
Stated admission probability&      -0.000\sym{***}&                     &                     &      -0.001\sym{***}\\
            &     (0.000)         &                     &                     &     (0.000)         \\
\textit{Academic achievements}                             &                 &                 &               &          \\
Eligibility score&                     &       0.002         &                     &       0.010\sym{***}\\
            &                     &     (0.001)         &                     &     (0.002)         \\
Middle school GPA&                     &      -0.001         &                     &      -0.001         \\
            &                     &     (0.002)         &                     &     (0.001)         \\
\textit{Demographic}                             &                 &                 &               &          \\ 
Age         &                     &       0.002         &                     &       0.001         \\
            &                     &     (0.001)         &                     &     (0.001)         \\
Female      &                     &      -0.001         &                     &      -0.003         \\
            &                     &     (0.005)         &                     &     (0.005)         \\
\textit{Socioeconomic factors}                             &                 &                 &               &          \\  
Income percentile, parents&                     &       0.004         &                     &       0.003         \\
            &                     &     (0.010)         &                     &     (0.010)         \\
\textit{Self-stated covariates}                             &                 &                 &               &          \\  
Confidence in own abilities&                     &                     &       0.000         &       0.000         \\
            &                     &                     &     (0.001)         &     (0.001)         \\
Risk profile&                     &                     &       0.001         &      -0.000         \\
            &                     &                     &     (0.001)         &     (0.001)         \\
Pessimistic &                     &                     &       0.002         &      -0.001         \\
            &                     &                     &     (0.005)         &     (0.005)         \\
Failed anticipation of cutoff movement&                     &                     &       0.007         &       0.009         \\
            &                     &                     &     (0.009)         &     (0.009)         \\
Willingness to postpone an additional year&                     &                     &      -0.008         &      -0.008         \\
            &                     &                     &     (0.005)         &     (0.005)         \\
Perceives rejection as failure&                     &                     &      -0.003         &      -0.003         \\
            &                     &                     &     (0.004)         &     (0.004)         \\
Difficult to comprehend admission process&                     &                     &       0.001         &      -0.002         \\
            &                     &                     &     (0.004)         &     (0.004)         \\
\hline
N           &    4,402        &    4,128      &    4,402       &    4,128         \\
Study program fixed effects&          Yes         &          Yes         &          Yes         &          Yes         \\
\hline\hline
\end{tabular}
}
\caption{Coefficient Results of Linear Probability Models for Payoff Relevant Mistake}
\label{tab:lin_reg_regretskip}
\floatfoot{Notes: The table shows results for four separate linear probability regression models. The table reports coefficient estimates and robust standard errors in parenthesis. Each equation consider payoff relevant mistake as an outcome variable. A payoff relevant mistake is defined as survey respondents (1) skips the impossible and (2) would have been admitted to the study program they state to have skipped. Survey respondents with missing data inputs are neglected in the regressions. Every equation include fixed effects for respondents' revealed first choice study program. \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\).}

\end{table}


==> tables/2020_udgaver/linreg_FE_regretskip_2021.tex <==
\begin{table}[]
\centering
\small
\renewcommand{\arraystretch}{1.25} 
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
 & \multicolumn{4}{c}{\textbf{Payoff relevant mistakes}} \\
 & (1) & (2) & (3) & (4) \\  
\hline
\multicolumn{5}{l}{\textit{Self-stated admission beliefs, favorite program} } \\
States zero admission probability&       0.008         &                     &                     &       0.009         \\
            &     (0.005)         &                     &                     &     (0.006)         \\
Stated admission probability&      -0.000\sym{***}&                     &                     &      -0.001\sym{***}\\
            &     (0.000)         &                     &                     &     (0.000)         \\
\textit{Academic achievements}                             &                 &                 &               &          \\
Eligibility score&                     &       0.001         &                     &       0.008\sym{***}\\
            &                     &     (0.001)         &                     &     (0.002)         \\
Middle school GPA&                     &      -0.002         &                     &      -0.002         \\
            &                     &     (0.001)         &                     &     (0.001)         \\
\textit{Demographic}                             &                 &                 &               &          \\ 
Age         &                     &       0.001         &                     &       0.001         \\
            &                     &     (0.001)         &                     &     (0.001)         \\
Female      &                     &      -0.002         &                     &      -0.004         \\
            &                     &     (0.003)         &                     &     (0.004)         \\
\textit{Socioeconomic factors}                             &                 &                 &               &          \\  
Income percentile, parents&                     &       0.007         &                     &       0.007         \\
            &                     &     (0.008)         &                     &     (0.008)         \\
Education length, parents&                     &      -0.001         &                     &      -0.001         \\
            &                     &     (0.001)         &                     &     (0.001)         \\
\textit{Self-stated covariates}                             &                 &                 &               &          \\  
Confidence in own abilities&                     &                     &      -0.001         &      -0.000         \\
            &                     &                     &     (0.001)         &     (0.001)         \\
Risk profile&                     &                     &       0.002\sym{**} &       0.001         \\
            &                     &                     &     (0.001)         &     (0.001)         \\
Pessimistic &                     &                     &       0.005         &       0.003         \\
            &                     &                     &     (0.004)         &     (0.004)         \\
Failed anticipation of cutoff movement&                     &                     &       0.008         &       0.009         \\
            &                     &                     &     (0.007)         &     (0.007)         \\
Willingness to postpone an additional year&                     &                     &      -0.004         &      -0.004         \\
            &                     &                     &     (0.004)         &     (0.004)         \\
Perceives rejection as failure&                     &                     &      -0.002         &      -0.002         \\
            &                     &                     &     (0.003)         &     (0.003)         \\
Difficult to comprehend admission process&                     &                     &       0.008\sym{*}  &       0.006         \\
            &                     &                     &     (0.003)         &     (0.003)         \\
\hline
N           &    8,643         &    8,078         &    8,643         &    8,078        \\
Study program fixed effects&         Yes         &         Yes         &         Yes         &         Yes         \\
Survey wave fixed effects &         Yes         &         Yes         &         Yes         &         Yes         \\
\hline\hline
\end{tabular}
}
\caption{Coefficient Results of Linear Probability Models for Payoff Relevant Mistake}
\label{tab:lin_reg_regretskip_2021}
\floatfoot{Notes: The table shows results for four separate linear probability regression models. The table reports coefficient estimates and robust standard errors in parenthesis. Each equation consider payoff relevant mistake as an outcome variable. \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\).}

\end{table}


==> tables/2020_udgaver/linreg_FE_skipimp.tex <==
\begin{table}[]
\centering
\small
\renewcommand{\arraystretch}{1.25} 
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
 & \multicolumn{4}{c}{\textbf{Skips the impossible}} \\
 & (1) & (2) & (3) & (4) \\  
\hline
\multicolumn{5}{l}{\textit{Self-stated admission beliefs, favorite program} } \\
States zero admission probability&       0.093\sym{***}&                     &                     &       0.085\sym{***}\\
            &     (0.021)         &                     &                     &     (0.021)         \\
Stated admission probability&      -0.002\sym{***}&                     &                     &      -0.002\sym{***}\\
            &     (0.000)         &                     &                     &     (0.000)         \\
\textit{Academic achievements}                             &                 &                 &               &          \\
Eligibility score&                     &      -0.044\sym{***}&                     &      -0.016\sym{***}\\
            &                     &     (0.004)         &                     &     (0.004)         \\
Middle school GPA&                     &       0.005         &                     &       0.004         \\
            &                     &     (0.004)         &                     &     (0.004)         \\
\textit{Demographic}                             &                 &                 &               &          \\ 
Age         &                     &       0.001         &                     &      -0.002         \\
            &                     &     (0.002)         &                     &     (0.002)         \\
Female      &                     &       0.003         &                     &      -0.015         \\
            &                     &     (0.012)         &                     &     (0.012)         \\
\textit{Socioeconomic factors}                             &                 &                 &               &          \\   
Income percentile, parents&                     &      -0.016         &                     &      -0.009         \\
            &                     &     (0.024)         &                     &     (0.023)         \\
\textit{Self-stated covariates}                             &                 &                 &               &          \\  
Confidence in own abilities&                     &                     &      -0.017\sym{***}&      -0.007\sym{*}  \\
            &                     &                     &     (0.003)         &     (0.003)         \\
Risk profile&                     &                     &       0.007\sym{**} &      -0.003         \\
            &                     &                     &     (0.003)         &     (0.003)         \\
Pessimistic &                     &                     &       0.060\sym{***}&       0.046\sym{***}\\
            &                     &                     &     (0.011)         &     (0.011)         \\
Failed anticipation of cutoff movement&                     &                     &       0.065\sym{*}  &       0.029         \\
            &                     &                     &     (0.025)         &     (0.025)         \\
Willingness to postpone an additional year&                     &                     &      -0.065\sym{***}&      -0.069\sym{***}\\
            &                     &                     &     (0.012)         &     (0.012)         \\
Perceives rejection as failure&                     &                     &       0.018         &       0.001         \\
            &                     &                     &     (0.010)         &     (0.010)         \\
Difficult to comprehend admission process&                     &                     &       0.020         &       0.020         \\
            &                     &                     &     (0.011)         &     (0.010)         \\
\hline
N           &    4,402        &    4,128      &    4,402       &    4,128         \\
Study program fixed effects&         Yes         &         Yes         &         Yes         &         Yes         \\
\hline\hline
\end{tabular}
}
\caption{Coefficient Results of Linear Probability Models for Skipping the Impossible}
\label{tab:lin_reg_res_FE_skipimp}
\floatfoot{Notes: The table shows results for four separate linear probability regression models. The table reports coefficient estimates and robust standard errors in parenthesis. Each equation consider skipping the impossible as an outcome variable. Skipping the impossible is defined as survey respondents who state they would select a different first priority study program if they could be enrolled at any study program. Survey respondents with missing data inputs are neglected in the regressions. Every equation include fixed effects for respondents' revealed first choice study program. \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\).}

\end{table}

==> tables/2020_udgaver/pop_vs_survey.tex <==
\begin{table}[!ht]
\centering\small
\begin{tabular}{lcccc} \hline \hline
Category          & Population Mean & Survey Mean & Reg Sample Mean & Pop vs. Survey \\ \hline
Age               & 22.0            & 21.7        & 20.6 & -0.30\sym{***}           \\
Women             & 0.55            & 0.64        & 0.64 & 0.09\sym{***}           \\
Eligibility Score & 8.25            & 8.63        & 8.81 & 0.38\sym{***}           \\
 &                 &             &          &      \\
\textit{Number of Choices} &                 &             &        &        \\
1                 & 0.40            & 0.36       & 0.26 & -0.04\sym{***}          \\
2                 & 0.24            & 0.23       & 0.21 & -0.01          \\
3                 & 0.16            & 0.16       & 0.18 & 0.00\sym{*}           \\
4                 & 0.10            & 0.12       & 0.14 & 0.02\sym{***}           \\
5                 & 0.05            & 0.06       & 0.08 & 0.01           \\
6                 & 0.03            & 0.03       & 0.05 & 0.00           \\
7                 & 0.02            & 0.02       & 0.03 & 0.00           \\
8                 & 0.01            & 0.02       & 0.05 & 0.01\sym{***}           \\ \hline
N                 & 48,796          & 7,344      & 4,128&                \\ \hline
\end{tabular}
\caption{Characteristics of Population and Survey Respondents}
\label{tab:pop_vs_survey}
\floatfoot{Notes: Means of indicator variables for sample universe and surveyed population. 'Population' is every student applying to higher education in Denmark in 2020. 'Survey' contains respondents who answered a population survey. Applicants received a survey invitation after the deadline of application to higher education. The survey was open for answers until the day before the announcement of cutoff levels. 'Reg Sample' includes the survey respondents included in the regression models. These are the survey respondents without missing data for covariates. 'Pop vs Survey' displays difference between population and survey mean. 'Age' is the age of subjects on January 1 2020. 'Number of Choices' presents count of study programs in students' submitted rank-ordered lists. P-values from a two-sided Welch's t-test is incated as \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\). }
\end{table}

==> tables/by_hypothesis/hyp_1_2_3_8_ols_no_fe.tex <==
\begin{table}[]
\centering
\small
\renewcommand{\arraystretch}{1.25} 
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{p{2cm}}}
\hline\hline
 & \multicolumn{2}{l}{\textbf{Reports}}  & \multicolumn{2}{l}{\textbf{Omits}} \\
  & \multicolumn{2}{l}{\textbf{non-truthfully}}  & \multicolumn{2}{l}{\textbf{most-preferred program}} \\
 & (1) & (2) & (3) & (4) \\  
\hline
\multicolumn{5}{l}{\textit{Hypothesis 1} } \\

Adm beliefs most-preferred program&      -0.271&            &      -0.270&            \\
            &     (0.019)&            &     (0.016)&            \\
Combined stated admission probability&            &      -0.325&            &      -0.327\\
            &            &     (0.022)&            &     (0.020)\\
\multicolumn{5}{l}{\textit{Hypothesis 2}} \\
Eligibility score&      -0.022&      -0.027&      -0.012&      -0.016\\
            &     (0.004)&     (0.004)&     (0.004)&     (0.004)\\
Middle school GPA&      -0.007&      -0.005&      -0.006&      -0.004\\
            &     (0.008)&     (0.008)&     (0.007)&     (0.007)\\
Age         &      -0.011&      -0.009&      -0.007&      -0.005\\
            &     (0.007)&     (0.007)&     (0.006)&     (0.005)\\
Female      &       0.033&       0.032&       0.005&       0.004\\
            &     (0.012)&     (0.012)&     (0.010)&     (0.010)\\
Income percentile, parents&      -0.005&      -0.005&      -0.010&      -0.010\\
            &     (0.007)&     (0.007)&     (0.006)&     (0.006)\\
Years of education, parents&       0.002&       0.003&       0.000&       0.001\\
            &     (0.007)&     (0.007)&     (0.006)&     (0.006)\\
\multicolumn{5}{l}{\textit{Hypothesis 3}} \\
Confidence in own abilities&      -0.001&       0.002&       0.008&       0.011\\
            &     (0.007)&     (0.007)&     (0.006)&     (0.006)\\
Risk willingness&      -0.013&      -0.012&      -0.019&      -0.018\\
            &     (0.007)&     (0.007)&     (0.006)&     (0.005)\\
Willingness to postpone an additional year&      -0.037&      -0.034&      -0.027&      -0.025\\
            &     (0.006)&     (0.006)&     (0.005)&     (0.005)\\
Perceives rejection as failure&      -0.009&      -0.010&      -0.011&      -0.012\\
            &     (0.006)&     (0.006)&     (0.005)&     (0.005)\\
Difficult to comprehend admission process&       0.025&       0.023&       0.017&       0.015\\
            &     (0.006)&     (0.006)&     (0.005)&     (0.005)\\
\multicolumn{5}{l}{\textit{Hypothesis 8} } \\
Understands strategy-proofness &      -0.032&      -0.032&      -0.034&      -0.034\\
            &     (0.014)&     (0.014)&     (0.011)&     (0.011)\\

\hline
N           &    3,767        &    3,767      &    3,767       &    3,767         \\
Study program fixed effects&         No         &         No         &         No         &         No         \\
\hline\hline
\end{tabular}
}
\caption{Coefficient Estimates of Robustness Analyses}
\label{tab:robust_reg_2021}
\floatfoot{Notes: Outcome variable of equations (1) and (2) is non-truthful reporting. Outcome variable of equations (3) and (4) is omitting most-preferred program. Robust standard errors are reported in parenthesis. The models are estimated on survey respondents from the 2021 wave, since the 2020 wave did not include the required questions.}

\end{table}

==> tables/by_hypothesis/hyp_1_2_3_ols_no_fe_nontruth.tex <==
\begin{table}[]
\centering
\small
\renewcommand{\arraystretch}{1.25} 
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
 & \multicolumn{4}{c}{\textbf{Reports non-truthfully}} \\
 & (1) & (2) & (3) & (4) \\                               
\hline
\multicolumn{5}{l}{\textit{Hypothesis 1} } \\
Adm beliefs most-preferred program                                    &      -0.299&            &            &      -0.243\\
                                                                      &     (0.011)&            &            &     (0.013)\\
\textit{Hypothesis 2}                             &                 &                 &               &          \\            
Eligibility score                                                     &            &      -0.048&            &      -0.023\\
                                                                      &            &     (0.003)&            &     (0.003)\\
Middle school GPA                                                     &            &       0.001&            &       0.001\\
                                                                      &            &     (0.006)&            &     (0.006)\\
Age                                                                   &            &       0.001&            &      -0.008\\
                                                                      &            &     (0.005)&            &     (0.005)\\
Female                                                                &            &       0.050&            &       0.011\\
                                                                      &            &     (0.009)&            &     (0.009)\\
Income percentile, parents                                            &            &      -0.002&            &      -0.001\\
                                                                      &            &     (0.005)&            &     (0.005)\\
Years of education, parents                                           &            &      -0.009&            &      -0.006\\
                                                                      &            &     (0.005)&            &     (0.005)\\
\textit{Hypothesis 3}                                      &                 &                 &               &          \\                 
Confidence in own abilities                                           &            &            &      -0.055&      -0.020\\
                                                                      &            &            &     (0.005)&     (0.005)\\
Risk willingness                                                      &            &            &       0.025&      -0.008\\
                                                                      &            &            &     (0.005)&     (0.005)\\
Willingness to postpone an additional year                            &            &            &      -0.040&      -0.041\\
                                                                      &            &            &     (0.005)&     (0.004)\\
Perceives rejection as failure                                        &            &            &       0.010&      -0.003\\
                                                                      &            &            &     (0.004)&     (0.004)\\
Difficult to comprehend admission process                             &            &            &       0.025&       0.023\\
                                                                      &            &            &     (0.004)&     (0.004)\\
\hline
N           &    8,049         &    8,049        &    8,049         &    8,049        \\
Study program fixed effects&         Yes         &         Yes         &         Yes         &         Yes         \\
Survey wave fixed effects &         Yes         &         Yes         &         Yes         &         Yes         \\
\hline\hline
\end{tabular}
}
\caption{Coefficient Results of Models for Non-truthful Reporting}
\label{tab:lin_reg_res_FE_nontruthful_2021}
\floatfoot{Notes: The table shows results for four separate linear probability regression models. The table reports coefficient estimates and robust standard errors in parenthesis. Each equation considers non-truthful reporting as an outcome variable.}

\end{table}

==> tables/by_hypothesis/hyp_1_2_3_ols_no_fe_omitprogram.tex <==
\begin{table}[]
\centering
\small
\renewcommand{\arraystretch}{1.25} 
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
 & \multicolumn{4}{c}{\textbf{Reports non-truthfully}} \\
 & (1) & (2) & (3) & (4) \\                               
\hline
\multicolumn{5}{l}{\textit{Hypothesis 1} } \\
Adm beliefs most-preferred program                                    &      -0.271&            &            &      -0.254\\
                                                                      &     (0.009)&            &            &     (0.011)\\
\textit{Hypothesis 2}                             &                 &                 &               &          \\            
Eligibility score                                                     &            &      -0.033&            &      -0.009\\
                                                                      &            &     (0.002)&            &     (0.003)\\
Middle school GPA                                                     &            &       0.001&            &       0.000\\
                                                                      &            &     (0.005)&            &     (0.005)\\
Age                                                                   &            &       0.005&            &      -0.003\\
                                                                      &            &     (0.004)&            &     (0.004)\\
Female                                                                &            &       0.026&            &      -0.008\\
                                                                      &            &     (0.007)&            &     (0.007)\\
Income percentile, parents                                            &            &      -0.000&            &      -0.001\\
                                                                      &            &     (0.004)&            &     (0.004)\\
Years of education, parents                                           &            &      -0.008&            &      -0.006\\
                                                                      &            &     (0.004)&            &     (0.004)\\
\textit{Hypothesis 3}                                      &                 &                 &               &          \\                 
Confidence in own abilities                                           &            &            &      -0.032&      -0.004\\
                                                                      &            &            &     (0.004)&     (0.004)\\
Risk willingness                                                      &            &            &       0.015&      -0.013\\
                                                                      &            &            &     (0.004)&     (0.004)\\
Willingness to postpone an additional year                            &            &            &      -0.028&      -0.030\\
                                                                      &            &            &     (0.004)&     (0.004)\\
Perceives rejection as failure                                        &            &            &       0.007&      -0.003\\
                                                                      &            &            &     (0.003)&     (0.003)\\
Difficult to comprehend admission process                             &            &            &       0.020&       0.018\\
                                                                      &            &            &     (0.004)&     (0.003)\\
\hline
N           &    8,049         &    8,049        &    8,049         &    8,049        \\
Study program fixed effects&         Yes         &         Yes         &         Yes         &         Yes         \\
Survey wave fixed effects &         Yes         &         Yes         &         Yes         &         Yes         \\
\hline\hline
\end{tabular}
}
\caption{Coefficient Results of Models for Omitting Most-preferred Program}
\label{tab:lin_reg_res_FE_skipimp_2021}
\floatfoot{Notes: The table shows results for four separate linear probability regression models. The table reports coefficient estimates and robust standard errors in parenthesis. Each equation considers omitting most-preferred program an outcome variable.}

\end{table}

==> tables/clogit_demand_reg.tex <==
\begin{table}[htbp]
\centering
\small
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
            &\multicolumn{1}{c}{Revealed Pref}&\multicolumn{1}{c}{Stated Pref}&\multicolumn{1}{c}{Stated Pref}\\
\hline
                        &            &            &            \\
Distance (1000 km)      &       -9.71&       -9.96&      -10.07\\
                        &      (0.18)&      (0.18)&      (0.18)\\
Program Peer Quality    &        9.43&       19.61&        7.50\\
                        &      (0.33)&      (0.43)&      (0.44)\\
Same Gender Share       &        2.26&        2.25&        2.30\\
                        &      (0.06)&      (0.06)&      (0.06)\\
Program Peer Parents Inc&        4.66&        5.55&        6.56\\
                        &      (0.65)&      (0.64)&      (0.61)\\
\hline
N                       &   6,888,528&   6,888,528&   5,973,743\\
Revealed Preferences    &         Yes&          No&          No \\
Truthful Assumption     &          No&          Yes&         No \\
Stability Assumption    &          No&          No&         Yes\\
\hline\hline
\end{tabular}
\caption{Comparison of demand models}
\label{tab:XXXX}
\floatfoot{Notes: This table provides regression coefficients from estimating demand models under the three approaches of (1) Revealed Preferences, (2) baseline model and (3) Using the stability assumption, see text for details. The models are estimated with standard errors clustered at the study program level. \emil{check lige teksten jeg fik skriblet sammen meget hurtigt}}
\end{table}


==> tables/clogit_res_2020.tex <==
begin{table}[htbp]
\centering
\small
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
            &\multicolumn{1}{c}{Revealed Pref}&\multicolumn{1}{c}{Stated Pref}&\multicolumn{1}{c}{Stated Pref}&\multicolumn{1}{c}{Revealed Pref}&\multicolumn{1}{c}{Stated Pref}&\multicolumn{1}{c}{Stated Pref}\\
\hline
        &            &            &            &            &            &            \\
Distance (1000 km)&       -9.53&       -9.58&       -9.74&       -9.59&       -9.69&       -9.79\\
            &      (0.23)&      (0.23)&      (0.23)&      (0.24)&      (0.24)&      (0.24)\\
Program Peer Quality&        9.27&        7.14&        9.54&       11.07&       27.49&       12.34\\
            &      (0.14)&      (0.12)&      (0.15)&      (0.49)&      (0.87)&      (0.76)\\
Same Gender Share&        1.73&        1.61&        1.79&        2.26&        2.27&        2.29\\
            &      (0.06)&      (0.06)&      (0.06)&      (0.08)&      (0.08)&      (0.09)\\
Program Peer Parents Inc&        3.80&        2.26&        4.02&        8.28&       10.42&       10.65\\
            &      (0.30)&      (0.27)&      (0.25)&      (1.13)&      (1.15)&      (1.10)\\
\hline
N           &   3,771,368&   3,771,368&   3,224,261&   3,771,368&   3,771,368&   3,224,261\\
Program FE  &          No&          No&          No&         Yes&         Yes&         Yes\\
Stability Assumption&          No&          No&         Yes&          No&          No&         Yes\\
\hline\hline
\end{tabular}
\caption{Conditional Logit Regressions...}
\label{tab:XXXX}
\floatfoot{Notes: ...}
\end{table}


==> tables/linreg_nontruthful.tex <==
\begin{table}[!ht]
\centering
\small
\renewcommand{\arraystretch}{1.25} 
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
 & \multicolumn{4}{c}{\textbf{Reports non-truthfully}} \\
 & (1) & (2) & (3) & (4) \\                               
\hline
\multicolumn{5}{l}{\textit{Self-stated admission beliefs, favorite program} } \\
States zero admission probability&       0.045\sym{*}  &                     &                     &       0.040         \\
            &     (0.023)         &                     &                     &     (0.023)         \\
Stated admission probability&      -0.003\sym{***}&                     &                     &      -0.002\sym{***}\\
            &     (0.000)         &                     &                     &     (0.000)         \\
\textit{Academic achievements}                             &                 &                 &               &          \\    
Eligibility score&                     &      -0.048\sym{***}&                     &      -0.020\sym{***}\\
            &                     &     (0.004)         &                     &     (0.004)         \\
Middle school GPA&                     &       0.004         &                     &       0.004         \\
            &                     &     (0.005)         &                     &     (0.005)         \\
\textit{Demographic}                             &                 &                 &               &          \\    
Age         &                     &       0.000         &                     &      -0.003         \\
            &                     &     (0.003)         &                     &     (0.003)         \\
Female      &                     &       0.033\sym{**} &                     &      -0.012         \\
            &                     &     (0.012)         &                     &     (0.012)         \\
\textit{Socioeconomic factors}                             &                 &                 &               &          \\  
Income percentile, parents&                     &      -0.034         &                     &      -0.022         \\
            &                     &     (0.027)         &                     &     (0.026)         \\
\textit{Self-stated covariates}                             &                 &                 &               &          \\     
Confidence in own abilities&                     &                     &      -0.029\sym{***}&      -0.017\sym{***}\\
            &                     &                     &     (0.003)         &     (0.003)         \\
Risk profile&                     &                     &       0.011\sym{***}&      -0.002         \\
            &                     &                     &     (0.003)         &     (0.003)         \\
Pessimistic &                     &                     &       0.042\sym{***}&       0.035\sym{**} \\
            &                     &                     &     (0.012)         &     (0.012)         \\
Failed anticipation of cutoff movement&                     &                     &       0.109\sym{***}&       0.076\sym{**} \\
            &                     &                     &     (0.028)         &     (0.029)         \\
Willingness to postpone an additional year&                     &                     &      -0.090\sym{***}&      -0.100\sym{***}\\
            &                     &                     &     (0.014)         &     (0.013)         \\
Perceives rejection as failure&                     &                     &       0.038\sym{***}&       0.009         \\
            &                     &                     &     (0.011)         &     (0.011)         \\
Difficult to comprehend admission process&                     &                     &       0.037\sym{**} &       0.035\sym{**} \\
            &                     &                     &     (0.013)         &     (0.012)         \\
\hline
N           &    4,402         &    4,128         &    4,402         &    4,128         \\
Study program fixed effects&          No         &          No         &          No         &          No         \\
\hline\hline
\end{tabular}
}
\caption{Coefficient Results of Linear Probability Models for Non-truthful Reporting - \textbf{Without fixed effects}}
\label{tab:lin_reg_res_nontruthful}
\floatfoot{Notes: The table shows results for four separate linear probability regression models. The table reports coefficient estimates and robust standard errors in parenthesis. Each equation consider non-truthful reporting as an outcome variable. Non-truthful reporting is defined as survey respondents who state they would change their submission if they could be enrolled at any study program. Survey respondents with missing data inputs are neglected in the regressions. Every equation include fixed effects for respondents' revealed first choice study program. \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\).}

\end{table}


==> tables/linreg_regretskip.tex <==
\begin{table}[!ht]
\centering
\small
\renewcommand{\arraystretch}{1.25} 
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
 & \multicolumn{4}{c}{\textbf{Payoff relevant mistakes}} \\
 & (1) & (2) & (3) & (4) \\  
\hline
\multicolumn{5}{l}{\textit{Self-stated admission beliefs, favorite program} } \\
States zero admission probability&       0.014         &                     &                     &       0.010         \\
            &     (0.008)         &                     &                     &     (0.008)         \\
Stated admission probability&      -0.000         &                     &                     &      -0.000\sym{*}  \\
            &     (0.000)         &                     &                     &     (0.000)         \\
\textit{Academic achievements}                             &                 &                 &               &          \\
Eligibility score&                     &       0.001         &                     &       0.003\sym{*}  \\
            &                     &     (0.001)         &                     &     (0.002)         \\
Middle school GPA&                     &      -0.002         &                     &      -0.002         \\
            &                     &     (0.001)         &                     &     (0.001)         \\
\textit{Demographic}                             &                 &                 &               &          \\ 
Age         &                     &       0.001         &                     &       0.001         \\
            &                     &     (0.001)         &                     &     (0.001)         \\
Female      &                     &      -0.012\sym{*}  &                     &      -0.014\sym{**} \\
            &                     &     (0.005)         &                     &     (0.005)         \\
\textit{Socioeconomic factors}                             &                 &                 &               &          \\  
Income percentile, parents&                     &       0.003         &                     &       0.003         \\
            &                     &     (0.009)         &                     &     (0.009)         \\
\textit{Self-stated covariates}                             &                 &                 &               &          \\  
Confidence in own abilities&                     &                     &       0.000         &      -0.000         \\
            &                     &                     &     (0.001)         &     (0.001)         \\
Risk profile&                     &                     &      -0.000         &      -0.001         \\
            &                     &                     &     (0.001)         &     (0.001)         \\
Pessimistic &                     &                     &       0.003         &       0.002         \\
            &                     &                     &     (0.004)         &     (0.004)         \\
Failed anticipation of cutoff movement&                     &                     &       0.004         &       0.003         \\
            &                     &                     &     (0.009)         &     (0.009)         \\
Willingness to postpone an additional year&                     &                     &      -0.010         &      -0.010         \\
            &                     &                     &     (0.005)         &     (0.005)         \\
Perceives rejection as failure&                     &                     &      -0.005         &      -0.005         \\
            &                     &                     &     (0.004)         &     (0.004)         \\
Difficult to comprehend admission process&                     &                     &       0.007         &       0.004         \\
            &                     &                     &     (0.005)         &     (0.005)         \\
\hline
N           &    4,402        &    4,128      &    4,402       &    4,128         \\
Study program fixed effects&          No         &          No         &          No         &          No         \\
\hline\hline
\end{tabular}
}
\caption{Coefficient Results of Linear Probability Models for Payoff Relevant Mistake - \textbf{Without fixed effects}}
\label{tab:lin_reg_regretskip}
\floatfoot{Notes: The table shows results for four separate linear probability regression models. The table reports coefficient estimates and robust standard errors in parenthesis. Each equation consider payoff relevant mistake as an outcome variable. A payoff relevant mistake is defined as survey respondents (1) skips the impossible and (2) would have been admitted to the study program they state to have skipped. Survey respondents with missing data inputs are neglected in the regressions.  \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\).}

\end{table}


==> tables/linreg_skipimp.tex <==
\begin{table}[]
\centering
\small
\renewcommand{\arraystretch}{1.25} 
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
 & \multicolumn{4}{c}{\textbf{Skips the impossible}} \\
 & (1) & (2) & (3) & (4) \\  
\hline
\multicolumn{5}{l}{\textit{Self-stated admission beliefs, favorite program} } \\
States zero admission probability&       0.093\sym{***}&                     &                     &       0.085\sym{***}\\
            &     (0.021)         &                     &                     &     (0.021)         \\
Stated admission probability&      -0.002\sym{***}&                     &                     &      -0.002\sym{***}\\
            &     (0.000)         &                     &                     &     (0.000)         \\
\textit{Academic achievements}                             &                 &                 &               &          \\
Eligibility score&                     &      -0.044\sym{***}&                     &      -0.016\sym{***}\\
            &                     &     (0.004)         &                     &     (0.004)         \\
Middle school GPA&                     &       0.005         &                     &       0.004         \\
            &                     &     (0.004)         &                     &     (0.004)         \\
\textit{Demographic}                             &                 &                 &               &          \\ 
Age         &                     &       0.001         &                     &      -0.002         \\
            &                     &     (0.002)         &                     &     (0.002)         \\
Female      &                     &       0.003         &                     &      -0.015         \\
            &                     &     (0.012)         &                     &     (0.012)         \\
\textit{Socioeconomic factors}                             &                 &                 &               &          \\   
Income percentile, parents&                     &      -0.016         &                     &      -0.009         \\
            &                     &     (0.024)         &                     &     (0.023)         \\
\textit{Self-stated covariates}                             &                 &                 &               &          \\  
Confidence in own abilities&                     &                     &      -0.017\sym{***}&      -0.007\sym{*}  \\
            &                     &                     &     (0.003)         &     (0.003)         \\
Risk profile&                     &                     &       0.007\sym{**} &      -0.003         \\
            &                     &                     &     (0.003)         &     (0.003)         \\
Pessimistic &                     &                     &       0.060\sym{***}&       0.046\sym{***}\\
            &                     &                     &     (0.011)         &     (0.011)         \\
Failed anticipation of cutoff movement&                     &                     &       0.065\sym{*}  &       0.029         \\
            &                     &                     &     (0.025)         &     (0.025)         \\
Willingness to postpone an additional year&                     &                     &      -0.065\sym{***}&      -0.069\sym{***}\\
            &                     &                     &     (0.012)         &     (0.012)         \\
Perceives rejection as failure&                     &                     &       0.018         &       0.001         \\
            &                     &                     &     (0.010)         &     (0.010)         \\
Difficult to comprehend admission process&                     &                     &       0.020         &       0.020         \\
            &                     &                     &     (0.011)         &     (0.010)         \\
\hline
N           &    4,402        &    4,128      &    4,402       &    4,128         \\
Study program fixed effects&         Yes         &         Yes         &         Yes         &         Yes         \\
\hline\hline
\end{tabular}
}
\caption{Coefficient Results of Linear Probability Models for Skipping the Impossible - Without fixed effects}
\label{tab:lin_reg_res_skipimp}
\floatfoot{Notes: The table shows results for four separate linear probability regression models. The table reports coefficient estimates and robust standard errors in parenthesis. Each equation consider skipping the impossible as an outcome variable. Skipping the impossible is defined as survey respondents who state they would select a different first priority study program if they could be enrolled at any study program. Survey respondents with missing data inputs are neglected in the regressions. Every equation include fixed effects for respondents' revealed first choice study program. \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\).}

\end{table}

==> tables/log_reg_regretskip.tex <==
\begin{table}[!ht]
\centering
\small
\renewcommand{\arraystretch}{1.25} 
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
 & \multicolumn{4}{c}{\textbf{Payoff relevant mistakes}} \\
 & (1) & (2) & (3) & (4) \\  
\hline
\multicolumn{5}{l}{\textit{Self-stated admission beliefs, favorite program} } \\
States zero admission probability&       0.540         &                     &                     &       0.395         \\
            &     (0.337)         &                     &                     &     (0.355)         \\
Stated admission probability&      -0.004         &                     &                     &      -0.011\sym{*}  \\
            &     (0.004)         &                     &                     &     (0.004)         \\
\textit{Academic achievements}                             &                 &                 &               &          \\
Eligibility score&                     &       0.060         &                     &       0.197\sym{*}  \\
            &                     &     (0.073)         &                     &     (0.087)         \\
Middle school GPA&                     &      -0.086         &                     &      -0.109         \\
            &                     &     (0.084)         &                     &     (0.087)         \\
\textit{Demographic}                             &                 &                 &               &          \\ 
Age         &                     &       0.065         &                     &       0.040         \\
            &                     &     (0.044)         &                     &     (0.046)         \\
Female      &                     &      -0.638\sym{**} &                     &      -0.790\sym{**} \\
            &                     &     (0.241)         &                     &     (0.252)         \\
\textit{Socioeconomic factors}                             &                 &                 &               &          \\  
Income percentile, parents&                     &       0.178         &                     &       0.190         \\
            &                     &     (0.552)         &                     &     (0.558)         \\
\textit{Self-stated covariates}                             &                 &                 &               &          \\  
Confidence in own abilities&                     &                     &       0.001         &      -0.005         \\
            &                     &                     &     (0.054)         &     (0.060)         \\
Risk profile&                     &                     &      -0.006         &      -0.070         \\
            &                     &                     &     (0.055)         &     (0.061)         \\
Pessimistic &                     &                     &       0.165         &       0.108         \\
            &                     &                     &     (0.234)         &     (0.252)         \\
Failed anticipation of cutoff movement&                     &                     &       0.242         &       0.213         \\
            &                     &                     &     (0.446)         &     (0.497)         \\
Willingness to postpone an additional year&                     &                     &      -0.487\sym{*}  &      -0.510\sym{*}  \\
            &                     &                     &     (0.231)         &     (0.246)         \\
Perceives rejection as failure&                     &                     &      -0.295         &      -0.268         \\
            &                     &                     &     (0.228)         &     (0.244)         \\
Difficult to comprehend admission process&                     &                     &       0.350         &       0.237         \\
            &                     &                     &     (0.230)         &     (0.247)         \\
\hline
N           &    4,402        &    4,128      &    4,402       &    4,128         \\
Study program fixed effects&          No         &          No         &          No         &          No         \\
\hline\hline
\end{tabular}
}
\caption{Coefficient Results of \textbf{Logit} Models for Payoff Relevant Mistakes}
\label{tab:logreg_regretskip}
\floatfoot{Notes: The table shows results for four separate logit regression models. The table reports coefficient estimates and robust standard errors in parenthesis. Each equation consider payoff relevant mistake as an outcome variable. A payoff relevant mistake is defined as survey respondents (1) skips the impossible and (2) would have been admitted to the study program they state to have skipped. Survey respondents with missing data inputs are neglected in the regressions. \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\).}

\end{table}


==> tables/log_reg_res_avg_mar_eff.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\small
\renewcommand{\arraystretch}{1.25} 
\begin{tabular}{lcccc} \hline \hline
                                                            & \multicolumn{2}{c}{Reports non-truthfully} & \multicolumn{2}{c}{Skips the impossible} \\
                                                            & (1)             & (2)                     & (3)              & (4)    \\  \hline
\textit{Academic achievements}                              &                 &                         &                  &                          \\                                                            
Eligibility score                                           & -0.0465         & -0.041                 &  -0.0328         &  -0.296             \\
                                                            & (0.004)         & (0.004)                 & (0.003)          & (0.003)                  \\
Middle School GPA                                          & 0.0023          & 0.0032                 & 0.008            & 0.013          \\
                                                            & (0.004)         & (0.004)                 & (0.003)          & (0.003)                  \\
\textit{Demographics}                                       &                 &                         &                  &                          \\
Age                                                         & -0.0017         & -0.0016                  & 0.0003          & 0.003              \\
                                                            & (0.002)         & (0.002)                 & (0.002)          & (0.002)                  \\
Female                                                      & 0.0382          & 0.0165                  & 0.0181           & 0.0061            \\
                                                            & (0.012)         & (0.012)                 & (0.010)          & (0.010)                  \\
\textit{Socioeconomic factors}                              &                 &                         &                  &                          \\
Income percentile, parents                                  & -0.0332         & -0.0153                  & 0.0001         &  0.0098            \\
                                                            & (0.026)         & (0.026)                 & (0.021)          & (0.021)                  \\
\textit{Self-stated covariates}                             &                 &                         &                  &                          \\
Confidence in own abilities                                 &                 & -0.0180                &                  & -0.0091            \\
                                                            &                 & (0.003)                 &                 & (0.002)                  \\
Risk profile                                                &                 & 0.0029                  &                   & 0.009             \\
                                                            &                 & (0.003)                 &                  & (0.002)                  \\
Pessimistic admission beliefs                               &                 & 0.0398                 &                  & 0.0326            \\
                                                            &                 & (0.012)                 &                 & (0.010)                  \\
Failed anticipation of cutoff movement                      &                  & 0.0532               &                   & 0.0234              \\
                                                            &                 & (0.026)                 &                  & (0.020)                  \\                                                            
\multirow{2}{5cm}{Willingness to postpone an additional year} &               & -0.0886                &                  & -0.0647          \\
                                                            &                 & (0.013)                 &                  & (0.011)                  \\
Perceive rejection as a failure                             &                 & 0.0090                  &                   & 0.0102               \\
                                                            &                 & (0.012)                 &                  & (0.009)                  \\
\multirow{2}{5cm}{Difficult to comprehend admission process}  &               & 0.0328                    &                   & 0.0269                  \\
                                                            &                 & (0.012)                 &                  & (0.010)                  \\ \hline
Study program fixed effects                                 & Yes             & Yes                     & Yes              & Yes                  \\              
N                                                           & 4,128           & 4,128                  & 4,128           & 4,128             \\ \hline \hline       
\end{tabular}
\caption{Average Marginal Effects in Logit Regressions}
\label{tab:log_reg_res_avg_marg_eff}
\floatfoot{Notes: The table shows results for four separate logit regressions. The table reports average marginal effects estimates and standard errors in parenthesis. The average marginal effects is the average marginal increase in probability of misreporting and skipping the impossible across every survey respondent Equation (1) and (2) consider non-truthful reporting as an outcome variable. Non-truthful reporting is defined as survey respondents who state they would change their submission if they could be enrolled at any study program. Equation (3) and (4) consider skipping the impossible as an outcome variable. Skipping the impossible is defined as survey respondents who state they would select a different first priority study program if they could be enrolled at any study program. The regressions are based on survey respondents for whom we have full data for. That is, survey respondents with missing data inputs are neglected in the regressions. Every equation include fixed effects for respondents' revealed first choice study program. Some study program fixed effects are excluded because they cause perfect multicollinarity.}
\end{table}

==> tables/log_reg_res_coefs.tex <==
\begin{table}[]
\centering
\small
\renewcommand{\arraystretch}{1.25} 
\begin{tabular}{lcccc} \hline \hline
                                                            & \multicolumn{2}{c}{Reports non-truthfully} & \multicolumn{2}{c}{Skips the impossible} \\
                                                            & (1)             & (2)                     & (3)              & (4)    \\  \hline
\textit{Academic achievements}                              &                 &                         &                  &                          \\                                                            
Eligibility score                                           & -0.3465         & -0.3165                 & -0.3828          & -0.3565              \\
                                                            & (0.028)         & (0.029)                 & (0.034)          & (0.035)                  \\
Middle School GPA                                          & 0.0169          & 0.0248                  &  0.0091          & 0.0151           \\
                                                            & (0.032)         & (0.033)                 & (0.040)          & (0.041)                  \\
\textit{Demographics}                                       &                 &                         &                  &                          \\
Age                                                         & -0.0124         & -0.0127                  &  0.0031          & 0.0035             \\
                                                            & (0.018)         & (0.019)                 & (0.022)          & (0.023)                  \\
Female                                                      & 0.2905          & 0.1287                  &  0.2153          & 0.0743           \\
                                                            & (0.094)         & (0.098)                 & (0.118)          & (0.123)                  \\
\textit{Socioeconomic factors}                              &                 &                         &                  &                          \\
Income percentile, parents                                  & -0.2474         & -0.1179                  &  0.0012         & 0.1183            \\
                                                            & (0.197)         & (0.201)                 & (0.246)          & (0.251)                  \\
\textit{Self-stated covariates}                             &                 &                         &                  &                          \\
Confidence in own abilities                                 &                 & -0.1393                 &                  & -0.1091            \\
                                                            &                 & (0.021)                 &                 & (0.026)                  \\
Risk profile                                                &                 & 0.0226                  &                   &  0.0108            \\
                                                            &                 & (0.022)                 &                  & (0.027)                  \\
Pessimistic admission beliefs                               &                 & 0.3049                 &                  &  0.3864           \\
                                                            &                 & (0.093)                 &                 & (0.116)                  \\
Failed anticipation of cutoff movement                      &                  & 0.3783                  &                   & 0.2626               \\
                                                            &                 & (0.171)                 &                  & (0.114)                  \\                                                            
\multirow{2}{5cm}{Willingness to postpone an additional year} &               & -0.6386                 &                  & -0.7118          \\
                                                            &                 & (0.092)                 &                  & (0.114)                  \\
Perceive rejection as a failure                             &                 & 0.0692                  &                   &  0.1232              \\
                                                            &                 & (0.090)                 &                  & (0.113)                  \\
\multirow{2}{5cm}{Difficult to comprehend admission process}  &               & 0.2491                    &                   & 0.3159                  \\
                                                            &                 & (0.090)                 &                  & (0.112)                  \\ \hline
Study program fixed effects                                 & Yes             & Yes                     & Yes              & Yes                  \\              
N                                                           & 4,128           & 4,128                  & 4,128           & 4,128             \\ \hline \hline       
\end{tabular}
\caption{Coefficient Results of Logit Regressions }
\label{tab:log_reg_res_coef}
\floatfoot{Notes: The table shows results for four separate logit regressions. The table reports coefficient estimates and standard errors in parenthesis. Equation (1) and (2) consider non-truthful reporting as an outcome variable. Non-truthful reporting is defined as survey respondents who state they would change their submission if they could be enrolled at any study program. Equation (3) and (4) consider skipping the impossible as an outcome variable. Skipping the impossible is defined as survey respondents who state they would select a different first priority study program if they could be enrolled at any study program. The regressions are based on survey respondents for whom we have full data for. That is, survey respondents with missing data inputs are neglected in the regressions. Every equation include fixed effects for respondents' revealed first choice study program. Some study program fixed effects are excluded because they cause perfect multicollinarity.}
\end{table}

==> tables/logreg_noFE.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
\hline
main        &                     &                     &                     &                     \\
High school GPA (=eligibility score)&      -0.311\sym{***}&      -0.280\sym{***}&      -0.311\sym{***}&      -0.289\sym{***}\\
            &    (0.0264)         &    (0.0277)         &    (0.0318)         &    (0.0332)         \\
Middle school GPA&      0.0192         &      0.0274         &      0.0162         &      0.0250         \\
            &    (0.0309)         &    (0.0316)         &    (0.0377)         &    (0.0383)         \\
Age         &    -0.00327         &    -0.00185         &      0.0185         &      0.0217         \\
            &    (0.0177)         &    (0.0183)         &    (0.0207)         &    (0.0213)         \\
Female      &       0.256\sym{**} &       0.126         &       0.186         &      0.0731         \\
            &    (0.0886)         &    (0.0924)         &     (0.109)         &     (0.113)         \\
Income percentile, parents&      -0.195         &     -0.0459         &      0.0273         &       0.180         \\
            &     (0.190)         &     (0.195)         &     (0.235)         &     (0.240)         \\
Confidence in own abilities&                     &      -0.132\sym{***}&                     &     -0.0986\sym{***}\\
            &                     &    (0.0203)         &                     &    (0.0245)         \\
Risk profile&                     &      0.0246         &                     &      0.0161         \\
            &                     &    (0.0212)         &                     &    (0.0257)         \\
Pessimistic &                     &       0.229\sym{**} &                     &       0.262\sym{*}  \\
            &                     &    (0.0889)         &                     &     (0.109)         \\
Failed anticipation of cutoff movement&                     &       0.354\sym{*}  &                     &       0.163         \\
            &                     &     (0.164)         &                     &     (0.202)         \\
Willingness to postpone an additional year&                     &      -0.646\sym{***}&                     &      -0.662\sym{***}\\
            &                     &    (0.0888)         &                     &     (0.107)         \\
Percives rejection as failure&                     &       0.126         &                     &       0.200         \\
            &                     &    (0.0874)         &                     &     (0.109)         \\
Difficult to comprehend admission process&                     &       0.262\sym{**} &                     &       0.339\sym{**} \\
            &                     &    (0.0875)         &                     &     (0.107)         \\
\hline
N           &        4128         &        4128         &        4128         &        4128         \\
Study program fixed effects&          No         &          No         &          No         &          No         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> tables/logreg_nontruthful.tex <==
\begin{table}[!ht]
\centering
\small
\renewcommand{\arraystretch}{1.25} 
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
 & \multicolumn{4}{c}{\textbf{Reports non-truthfully}} \\
 & (1) & (2) & (3) & (4) \\                               
\hline
\multicolumn{5}{l}{\textit{Self-stated admission beliefs, favorite program} } \\
 &                     &                     &                     &                     \\
States zero admission probability&       0.058         &                     &                     &       0.026         \\
            &     (0.110)         &                     &                     &     (0.121)         \\
Stated admission probability&      -0.021\sym{***}&                     &                     &      -0.018\sym{***}\\
            &     (0.001)         &                     &                     &     (0.002)         \\
\textit{Academic achievements}                             &                 &                 &               &          \\     
Eligibility score&                     &      -0.311\sym{***}&                     &      -0.145\sym{***}\\
            &                     &     (0.026)         &                     &     (0.030)         \\
Middle school GPA&                     &       0.019         &                     &       0.020         \\
            &                     &     (0.031)         &                     &     (0.033)         \\
\textit{Demographic}                             &                 &                 &               &          \\         
Age         &                     &      -0.003         &                     &      -0.024         \\
            &                     &     (0.018)         &                     &     (0.019)         \\
Female      &                     &       0.256\sym{**} &                     &      -0.062         \\
            &                     &     (0.089)         &                     &     (0.096)         \\
\textit{Socioeconomic factors}                             &                 &                 &               &          \\ 
Income percentile, parents&                     &      -0.195         &                     &      -0.151         \\
            &                     &     (0.190)         &                     &     (0.200)         \\
\textit{Self-stated covariates}                             &                 &                 &               &          \\   
Confidence in own abilities&                     &                     &      -0.183\sym{***}&      -0.112\sym{***}\\
            &                     &                     &     (0.018)         &     (0.021)         \\
Risk profile&                     &                     &       0.077\sym{***}&      -0.012         \\
            &                     &                     &     (0.020)         &     (0.022)         \\
Pessimistic &                     &                     &       0.296\sym{***}&       0.279\sym{**} \\
            &                     &                     &     (0.083)         &     (0.092)         \\
Failed anticipation of cutoff movement&                     &                     &       0.678\sym{***}&       0.536\sym{**} \\
            &                     &                     &     (0.149)         &     (0.169)         \\
Willingness to postpone an additional year&                     &                     &      -0.581\sym{***}&      -0.741\sym{***}\\
            &                     &                     &     (0.083)         &     (0.092)         \\
Perceives rejection as failure&                     &                     &       0.271\sym{***}&       0.067         \\
            &                     &                     &     (0.082)         &     (0.090)         \\
Difficult to comprehend admission process&                     &                     &       0.248\sym{**} &       0.269\sym{**} \\
            &                     &                     &     (0.082)         &     (0.090)         \\
\hline
N           &    4,402         &    4,128        &    4,402         &    4,128         \\
Study program fixed effects&          No         &          No         &          No         &          No         \\
\hline\hline
\end{tabular}
}
\caption{Coefficient Results of \textbf{Logit} Models for Non-truthful Reporting}
\label{tab:logreg_nontruthful}
\floatfoot{Notes: The table shows results for four separate logit regression models. The table reports coefficient estimates and robust standard errors in parenthesis. Each equation consider non-truthful reporting as an outcome variable. Non-truthful reporting is defined as survey respondents who state they would change their submission if they could be enrolled at any study program. Survey respondents with missing data inputs are neglected in the regressions. Every equation include fixed effects for respondents' revealed first choice study program. \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\).}

\end{table}

==> tables/logreg_skipimp.tex <==
\begin{table}[!ht]
\centering
\small
\renewcommand{\arraystretch}{1.25} 
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
 & \multicolumn{4}{c}{\textbf{Skips the impossible}} \\
 & (1) & (2) & (3) & (4) \\  
\hline
\multicolumn{5}{l}{\textit{Self-stated admission beliefs, favorite program} } \\
&                     &                     &                     &                     \\
States zero admission probability&       0.151         &                     &                     &       0.092         \\
            &     (0.127)         &                     &                     &     (0.138)         \\
Stated admission probability&      -0.034\sym{***}&                     &                     &      -0.034\sym{***}\\
            &     (0.002)         &                     &                     &     (0.003)         \\
\textit{Academic achievements}                             &                 &                 &               &          \\
Eligibility score&                     &      -0.311\sym{***}&                     &      -0.067         \\
            &                     &     (0.032)         &                     &     (0.038)         \\
Middle school GPA&                     &       0.016         &                     &       0.002         \\
            &                     &     (0.038)         &                     &     (0.041)         \\
\textit{Demographic}                             &                 &                 &               &          \\ 
Age         &                     &       0.018         &                     &      -0.017         \\
            &                     &     (0.021)         &                     &     (0.023)         \\
Female      &                     &       0.186         &                     &      -0.244\sym{*}  \\
            &                     &     (0.109)         &                     &     (0.121)         \\
\textit{Socioeconomic factors}                             &                 &                 &               &          \\ 
Income percentile, parents&                     &       0.027         &                     &       0.009         \\
            &                     &     (0.235)         &                     &     (0.253)         \\
\textit{Self-stated covariates}                             &                 &                 &               &          \\ 
Confidence in own abilities&                     &                     &      -0.154\sym{***}&      -0.068\sym{**} \\
            &                     &                     &     (0.022)         &     (0.026)         \\
Risk profile&                     &                     &       0.075\sym{**} &      -0.039         \\
            &                     &                     &     (0.024)         &     (0.027)         \\
Pessimistic &                     &                     &       0.335\sym{**} &       0.335\sym{**} \\
            &                     &                     &     (0.103)         &     (0.117)         \\
Failed anticipation of cutoff movement&                     &                     &       0.583\sym{**} &       0.450\sym{*}  \\
            &                     &                     &     (0.182)         &     (0.215)         \\
Willingness to postpone an additional year&                     &                     &      -0.573\sym{***}&      -0.835\sym{***}\\
            &                     &                     &     (0.101)         &     (0.116)         \\
Perceives rejection as failure&                     &                     &       0.350\sym{***}&       0.142         \\
            &                     &                     &     (0.102)         &     (0.115)         \\
Difficult to comprehend admission process&                     &                     &       0.305\sym{**} &       0.352\sym{**} \\
            &                     &                     &     (0.100)         &     (0.113)         \\
\hline
N           &    4,402        &    4,128      &    4,402       &    4,128         \\
Study program fixed effects&          No         &          No         &          No         &          No         \\
\hline\hline
\end{tabular}
}
\caption{Coefficient Results of \textbf{Logit} Models for Skipping the Impossible}
\label{tab:logreg_skipimp}
\floatfoot{Notes: The table shows results for four separate logit probability regression models. The table reports coefficient estimates and robust standard errors in parenthesis. Each equation consider skipping the impossible as an outcome variable. Skipping the impossible is defined as survey respondents who state they would select a different first priority study program if they could be enrolled at any study program. Survey respondents with missing data inputs are neglected in the regressions. Every equation include fixed effects for respondents' revealed first choice study program. \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\).}

\end{table}


==> tables/reg_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\small
\renewcommand{\arraystretch}{1.25} 
\begin{tabular}{lcccc} \hline \hline
                                                            & \multicolumn{2}{c}{Coefficient Estimates} & \multicolumn{2}{c}{Average Marginal Effects} \\
                                                            & (Misreporting)             & (Skips impossible)                     & (Misreporting)              & (Skips impossible)    \\  \hline
Eligibility score                                           & -0.2803         & -0.2891                 & -0.0379          & -0.0259                  \\
                                                            & (0.028)         & (0.033)                 & (0.004)          & (0.003)                  \\
Primary School GPA                                          & 0.0273          & 0.0251                  & 0.0037           & 0.0023                   \\
                                                            & (0.032)         & (0.038)                 & (0.004)          & (0.003)                  \\
\textit{Demographics}                                       &                 &                         &                  &                          \\
Age                                                         & -0.0018         & 0.0215                  & -0.0002          & 0.0019                   \\
                                                            & (0.018)         & (0.021)                 & (0.002)          & (0.002)                  \\
Female                                                      & 0.1256          & 0.0731                  & 0.0161           & 0.0065                   \\
                                                            & (0.092)         & (0.113)                 & (0.012)          & (0.010)                  \\
\textit{Socioeconomic factors}                              &                 &                         &                  &                          \\
Income percentile, mom                                      & -0.0055         & -0.0691                 & -0.0007          & -0.0062                  \\
                                                            & (0.155)         & (0.190)                 & (0.021)          & (0.017)                  \\
Income percentile, dad                                      & -0.0402         & 0.2484                  & -0.0054          & 0.0222                   \\
                                                            & (0.154)         & (0.191)                 & (0.021)          & (0.017)                  \\
\textit{Self-stated covariates}                             &                 &                         &                  &                          \\
Confidence in own abilities                                 & -0.1318         & -0.0993                 & -0.0178          & -0.0089                  \\
                                                            & (0.020)         & (0.024)                 & (0.003)          & (0.002)                  \\
Risk profile                                                & 0.0246          & 0.0159                  & 0.0033           & 0.0014                   \\
                                                            & (0.021)         & (0.026)                 & (0.003)          & (0.002)                  \\
Pessimistic admission beliefs                               & 0.2290          & 0.2642                  & 0.0312           & 0.0238                   \\
                                                            & (0.089)         & (0.109)                 & (0.012)          & (0.010)                  \\
Failed anticipation of cutoff movement                      & 0.3539          & 0.1621                  & 0.0519           & 0.0152                   \\
                                                            & (0.164)         & (0.202)                 & (0.026)          & (0.020)                  \\                                                            
\multirow{2}{5cm}{Willingness to postpone an additional year} & -0.6467       & -0.6600                 & -0.0941          & -0.0645                  \\
                                                            & (0.089)         & (0.107)                 & (0.014)          & (0.011)                  \\
Percept rejection as a failure                              & 0.1260          & 0.1987                  & 0.0170           & 0.0176                   \\
                                                            & (0.087)         & (0.109)                 & (0.012)          & (0.001)                  \\
\multirow{2}{5cm}{Difficult to comprehent admission process}  & 0.2620        & 0.3382                  & 0.0362           & 0.0312                   \\
                                                            & (0.087)         & (0.107)                 & (0.012)          & (0.010)                  \\ \hline
N                                                           & 4,128           & 4,128                  & 4,128           & 4,128             \\ \hline \hline       
\end{tabular}
\caption{Logit Regression Results}
\label{tab:reg_res}
\floatfoot{Notes: The table shows results for two separate logit regressions. The first regression considers misreporting as an outcome variable. Misreporting is defined as survey respondents who state they would change their submission if they could be enrolled at any study program. The second regression considers skipping the impossible. Skipping the impossible is defined as survey respondents who state they would select a different first priority study program if they could be enrolled at any study program. The regressions are based on survey respondents for whom we have full data for. That is, survey respondents with missing data inputs are neglected in the regressions. The table report coefficient estimates and average marginal effects. The average marginal effects is the average marginal increase in probability of misreporting and skipping the impossible across every survey respondent. Standard errors are shown in parenthesis.}
\end{table}

==> tables/robust_bint_reg_vars_ntruth.tex <==
\begin{table}[]
\centering
\small
\renewcommand{\arraystretch}{1.25} 
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\hline\hline
 & \multicolumn{6}{c}{\textbf{Reports Non-truthfully}} \\
 & (1) & (2) & (3) & (4) & (5) & (6)\\  
\hline
Stated admission probability                      &      -0.343&      -0.232&      -0.231&      -0.231&      -0.232&      -0.233\\
                                                  &     (0.057)&     (0.017)&     (0.017)&     (0.023)&     (0.017)&     (0.017)\\
Eligibility score                                 &      -0.031&      -0.025&      -0.026&      -0.026&      -0.025&      -0.025\\
                                                  &     (0.005)&     (0.004)&     (0.004)&     (0.004)&     (0.004)&     (0.004)\\
Middle school GPA                                 &      -0.000&      -0.008&       0.001&       0.001&       0.000&       0.000\\
                                                  &     (0.006)&     (0.010)&     (0.006)&     (0.006)&     (0.006)&     (0.006)\\
Age                                               &      -0.011&      -0.010&      -0.013&      -0.010&      -0.010&      -0.010\\
                                                  &     (0.005)&     (0.005)&     (0.007)&     (0.005)&     (0.005)&     (0.005)\\
Female                                            &       0.009&       0.008&       0.009&       0.009&       0.008&       0.008\\
                                                  &     (0.010)&     (0.010)&     (0.010)&     (0.019)&     (0.010)&     (0.010)\\
Income percentile, parents                        &      -0.002&      -0.002&      -0.002&      -0.002&      -0.009&      -0.002\\
                                                  &     (0.005)&     (0.005)&     (0.005)&     (0.005)&     (0.009)&     (0.005)\\
Education length, parents                         &      -0.007&      -0.007&      -0.007&      -0.007&      -0.007&      -0.019\\
                                                  &     (0.005)&     (0.005)&     (0.005)&     (0.005)&     (0.005)&     (0.009)\\
Confidence in own abilities                       &      -0.021&      -0.021&      -0.020&      -0.020&      -0.020&      -0.020\\
                                                  &     (0.005)&     (0.005)&     (0.005)&     (0.005)&     (0.005)&     (0.005)\\
Risk willingness                                  &      -0.010&      -0.010&      -0.010&      -0.010&      -0.010&      -0.010\\
                                                  &     (0.005)&     (0.005)&     (0.005)&     (0.005)&     (0.005)&     (0.005)\\
Willingness to postpone an additional year        &      -0.038&      -0.038&      -0.038&      -0.038&      -0.038&      -0.038\\
                                                  &     (0.004)&     (0.004)&     (0.004)&     (0.004)&     (0.004)&     (0.004)\\
Perceives rejection as failure                    &      -0.004&      -0.004&      -0.004&      -0.004&      -0.004&      -0.004\\
                                                  &     (0.004)&     (0.004)&     (0.004)&     (0.004)&     (0.004)&     (0.004)\\
Difficult to comprehend admission process         &       0.020&       0.020&       0.020&       0.020&       0.020&       0.020\\
                                                  &     (0.004)&     (0.004)&     (0.004)&     (0.004)&     (0.004)&     (0.004)\\
Eligibility score X Beliefs                               &       0.012&            &            &            &            &            \\
                                                  &     (0.006)&            &            &            &            &            \\
Middle school GPA X Beliefs                       &            &       0.016&            &            &            &            \\
                                                  &            &     (0.012)&            &            &            &            \\
Age X Beliefs                                     &            &            &       0.008&            &            &            \\
                                                  &            &            &     (0.010)&            &            &            \\
Female X Beliefs                                  &            &            &            &       0.000&            &            \\
                                                  &            &            &            &     (0.023)&            &            \\
Parents' Income Rank X Beliefs&                   &            &            &            &       0.013&            \\
                                                  &            &            &            &            &     (0.011)&            \\
Parents' Years of Education X Beliefs             &            &            &            &            &            &       0.024\\
                                                  &            &            &            &            &            &     (0.011)\\
\hline
N           &    8,078         &    8,078         &    8,078         &    8,078    &   8,078 & 8,078  \\
Study program fixed effects&         Yes         &         Yes         &         Yes         &         Yes    & Yes   & Yes  \\
Survey wave fixed effects &         Yes         &         Yes         &         Yes         &         Yes    & Yes  & Yes    \\
\hline\hline
\end{tabular}
}
\caption{Coefficient Results of Models with Stated Admission Probability Interactions}
\label{tab:robust_bint_reg_vars_ntruth}
\floatfoot{}

\end{table}

==> tables/within_std_prgm_cutoff_std.tex <==
\begin{table}[]
\centering
\begin{tabular}{cccccc} \hline \hline
Average & Minimum & 1st Quartile & Median & 3rd Quartile & Maximum \\ \hline 
0.9        & 0       & 0            & 0.5    & 1.4          & 4.7    \\ \hline
\end{tabular}
\caption{Within Study Program Standard Deviation of Cutoff Level}
\label{tab:within_stud_program_cutoff_std}
\end{table}
